Sparse IDMA: A Joint Graph-Based Coding Scheme for Unsourced Random Access

This article introduces a novel communication paradigm for the unsourced, uncoordinated Gaussian multiple access problem. The major components of the envisioned framework are as follows. The encoded bits of every message are partitioned into two groups. The first portion is transmitted using a compressive sensing scheme, whereas the second set of bits is conveyed using a multi-user coding scheme. The compressive sensing portion is key in sidestepping some of the challenges posed by the unsourced aspect of the problem. The information afforded by the compressive sensing is employed to create a sparse random multi-access graph conducive to joint decoding. This construction leverages the lessons learned from traditional IDMA into creating low-complexity schemes for the unsourced setting and its inherent randomness. Under joint message-passing decoding, the proposed scheme offers comparable performance to existing low-complexity alternatives. Findings are supported by numerical simulations.

==> Figures/polar_decoder.tex <==
\tikzstyle{cnode}=[circle,minimum size=0.75cm,draw]%,fill=blue!25]
\tikzstyle{cgnode}=[circle,draw]%,fill=blue!25]
\tikzstyle{crnode}=[circle,draw]%,fill=blue!25]
\tikzstyle{conode}=[rectangle,draw,fill=black!15]
\tikzstyle{cpnode}=[circle,draw]%,fill=blue!25]
\tikzstyle{pnode}=[circle,draw,fill=black,inner sep=1.5pt]
\tikzstyle{rnode}=[rectangle,draw,outer sep=0pt]%,fill=red!50]
\tikzstyle{fnode}=[rectangle,draw,minimum height=0.6cm,minimum width=1.1cm,fill=red!75,text centered]
\tikzstyle{prnode}=[rectangle,minimum height=0.6cm,minimum width=1.1cm,text centered,draw]
\tikzstyle{block}=[rectangle,draw,minimum width=2cm,minimum height=1cm,text centered]
\tikzstyle{bigblock}=[rectangle,draw,minimum width=2cm,minimum height=3cm,text centered]
\tikzstyle{dummyblock}=[rectangle,minimum width=2cm,minimum height=3cm,text centered]
\tikzstyle{sblock}=[rectangle,draw,minimum width=1cm,minimum height=1cm,text centered]
\tikzstyle{prnodesimple}=[rectangle,draw,text width=11em,text centered,outer sep=0pt]
\tikzstyle{bigsnake}=[snake=snake,segment amplitude=4mm, segment length=4mm, line after snake=5mm]
\tikzstyle{smallsnake}=[snake=snake,segment amplitude=0.7mm, segment length=4mm, line after snake=3mm]

\begin{tikzpicture}[every node/.style={scale=1}]
\begin{scope}[node distance=2cm,>=angle 90,semithick]
\node (input1) {};
\node (input2) [below of=input1,xshift=0cm,yshift=0.3cm] {};
\node[cpnode] (adder) [right of=input1,xshift=2cm,yshift=0cm] {$\oplus$};
\node[pnode] (nop) [right of=input2,xshift=2cm,yshift=0cm]{};
\node (op1) [right of=adder]{};
\node (op2) [right of=nop]{};
\only<1>{\draw (adder) -- node[above]{$d(2,1) \in \mathbb{F}_4$} (op1);
\draw (nop) --  node[above]{$d(2,2) \in \mathbb{F}_4$} (op2);
\draw (adder) -- node[above]{$d(1,1) \in \mathbb{F}_4$} (input1);
\draw (nop) -- node[above]{$d(1,2) \in \mathbb{F}_4$} (input2);
\draw (nop.270)--   (adder.270);}
\only<2>{\draw (adder) -- node[above]{$\underbar P_{d(2,1)}$} (op1);
\draw (nop) --  node[above]{$\underbar P_{d(2,2)}$} (op2);
\draw (adder) -- node[above]{} (input1);
\draw (nop) -- node[above]{} (input2);
\draw (nop.270)--   (adder.270);}
\only<3>{\draw (adder) -- node[above]{$\underbar {P}_{d(2,1)}$} (op1);
\draw (nop) --  node[above]{$\underbar  {P}_{d(2,2)}$} (op2);
\draw (adder) -- node[above]{$\underbar {P}_{d(2,1)} \circledast \underbar {P}_{d(2,2)}$} (input1);
\draw (nop) -- node[above]{} (input2);
\draw (nop.270)--   (adder.270);}
%\only<4>{\draw (adder) -- node[above]{$\underbar {P}_{d(2,1)} \circledast \underbar {P}_{d(2,2)}$} (input1);}
\onslide<4->{\draw (adder) -- node[above]{$\underbar {P}_{d(2,1)}$} (op1);
\draw (nop) --  node[above]{$\underbar  {P}_{d(2,2)}$} (op2);
\draw (nop.270)--   (adder.270);
\draw (nop) -- node[above]{} (input2);
\draw (adder) -- node[above]{$\widehat{d}(1,1)$} (input1);}
\only<5->{\draw (nop) -- node[above]{$\underbar{P}_{\widehat{d}(1,1)\oplus d(2,1)} \odot \underbar{P}_{d(2,2)}$} (input2);}
\end{scope}
\end{tikzpicture} 

==> Figures/preamble_beamer.tex <==
\usepackage{amsmath,amssymb,amsthm}
\usepackage{enumerate}
\usepackage{stfloats}
\usepackage{comment}
\usepackage{subfig}
\usepackage{graphicx}
\usepackage{color}
\usepackage{tikz}
\usetikzlibrary{%
  arrows,%
  calc,
  decorations,%decorations
  decorations.markings,
  decorations.pathmorphing,
  shapes.misc,% wg. rounded rectangle
  shapes.arrows,%
  shapes.callouts, %
  shapes,%
  chains,%
  matrix,%
  positioning,% wg. " of "
  patterns,% slanted lines fill
  scopes,%
  petri,%
  fadings
}

%\usepackage{enumitem}
\usepackage{pgfplots}
\pgfplotsset{compat=1.3}
\usepgflibrary{shapes}


\usepackage[T1]{fontenc}
%\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage[mathscr]{euscript}



\setbeamertemplate{itemize item}[triangle]
\setbeamertemplate{itemize subitem}[circle]
\setbeamertemplate{itemize subsubitem}{$-$}

\setbeamertemplate{blocks}[rounded,shadow=true]
\setbeamercolor{block title}{fg=black,bg=blue!30!white}
\setbeamercolor{block body}{fg=black,bg=blue!10!white}

\newenvironment<>{defn}[1]{%
  \setbeamertemplate{blocks}[default]%
  \setbeamercolor{block title}{fg=blue,bg=white}%
  \setbeamercolor{block body}{fg=black,bg=white}%
  \begin{block}#2{#1}}{\end{block}}

\setbeamerfont{alerted text}{family=\sffamily, shape=\slshape}
\setbeamercolor{alerted text}{fg=red!95!white}


\newcommand{\indicator}[1]{\mathbbm{1}_{\left\{ {#1} \right\} }}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}

\newcommand{\defeq}{\triangleq}
\newcommand{\Pp}{\mathbb{P}}
\newcommand{\Gm}{\mathbf{G}}
\newcommand{\Hm}{\mathbf{H}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zp}{\mathbb{Z}_{+}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rp}{\R_{+}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Zw}{\mathbb{Z}[\omega]}
\newcommand{\Zi}{\mathbb{Z}[i]}
\newcommand{\mc}{\mathcal}
\newcommand{\mbb}{\mathbb}

\newcommand{\av}{\underline{a}}
\newcommand{\wv}{\underline{w}}
\newcommand{\cv}{\underline{c}}
\newcommand{\ev}{\underline{e}}
\newcommand{\sv}{\underline{s}}
\newcommand{\xv}{\underline{x}}
\newcommand{\bv}{\underline{b}}
\newcommand{\kv}{\underline{k}}
\newcommand{\zv}{\underline{z}}
\newcommand{\yv}{\underline{y}}
\newcommand{\hv}{\underline{h}}
\newcommand{\rv}{\underline{r}}

\newcommand{\Yv}{\underline{Y}}
\newcommand{\Xv}{\underline{X}}
\newcommand{\Rv}{\underline{R}}
\newcommand{\mfk}[1]{\mathfrak{#1}}

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\newcommand{\wpdash}{w^\mathrm{p}}
\newcommand{\wc}{w^\mathrm{c}}


%\newcommand{\mb}[1]{\mathbf{#1}}
%\newcommand{\mbb}[1]{\mathbb{#1}}
%\newcommand{\mr}[1]{\mathrm{#1}}
%\newcommand{\mc}[1]{\mathcal{#1}}
%\newcommand{\mfk}[1]{\mathfrak{#1}}
%
%\newcommand{\av}{\vec{\mathrm{a}}}
%\newcommand{\bv}{\vec{\mathrm{b}}}
%\newcommand{\cv}{\vec{\mathrm{c}}}
%\newcommand{\hv}{\vec{\mathrm{h}}}
%\newcommand{\xv}{\vec{\mathrm{x}}}
%\newcommand{\yv}{\vec{\mathrm{y}}}
%\newcommand{\zv}{\vec{\mathrm{z}}}
%
%
%\newcommand{\wpdash}{w^\mathrm{p}}
%\newcommand{\wc}{w^\mathrm{c}}


%\newcommand{\defeq}{\triangleq}
%\newcommand{\Pp}{\mathbb{P}}
%\newcommand{\E}{\mathbb{E}}
%\newcommand{\N}{\mathbb{N}}
%\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\Zp}{\mathbb{Z}_{+}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\Rp}{\R_{+}}
%\newcommand{\C}{\mathbb{C}}
%\newcommand{\Q}{\mathbb{Q}}
%\newcommand{\F}{\mathbb{F}}
%\newcommand{\Zw}{\mathbb{Z}[\omega]}
%\newcommand{\Zi}{\mathbb{Z}[i]}

%\newcommand{\wv}{\underline{w}}
%\newcommand{\cv}{\underline{c}}
%\newcommand{\xv}{\underline{x}}
%\newcommand{\kv}{\underline{k}}
%\newcommand{\zv}{\underline{z}}
%\newcommand{\yv}{\underline{y}}
%\newcommand{\hv}{\underline{h}}


\def\Ktot{K_{\text{tot}}}
\def\Ka{K_{\text{a}}}
\def \Mp{M_{\mathrm{p}}}
\def \Mc{M_{\mathrm{c}}}

\def \Np{N_{\mathrm{p}}}
\def \Nc{N_{\mathrm{c}}}
\def \Pp{P_{\mathrm{p}}}
\def \Pc{P_{\mathrm{c}}}
\def \Bp{B_{\mathrm{p}}}
\def \Bc{B_{\mathrm{c}}}

\def\dmin{d_{\mathrm{min}}}
\def\dmax{d_{\mathrm{max}}}
\def\wmin{w_{\text{min}}}
\def\wmax{w_{\text{max}}}
\def\Pr{\mathrm{Pr}}

\DeclareMathOperator*{\argmin}{\,arg\ min}
\DeclareMathOperator*{\argmax}{\,arg\ max}
\newcommand{\coleq}{\mathrel{\mathop:}=} 

==> numericalresults.tex <==
\section{Numerical Results}
{\color{red} Need to be rewritten}
We pick the same parameters as in \cite{ordentlich2017low}. 
\begin{itemize}
\item Number of bits each user intends to transmit $B=100$
\item Total number of channel uses $N=30000$
\item Total number of active users $\Ka\in [25:300]$ 
\item Maximum per user error probability $P_e\leq \epsilon=0.05$.
\end{itemize}
\subsection*{Compressed Sensing}
We choose $\Bp=14$ and $\Np=1500$ and we choose $\Np$ random rows of Fourier matrix of dimension $2^{Bp}$ as the choice of our sensing matrix $\mathbf{A}$. This implies the parameters for channel coding are $\Bc=86$ and $\Nc=28500$. For the choice  


In Fig.~\ref{fig:simulationresults30000} the curves labelled $T=2$, $T=4$ correspond to the performance of our proposed scheme assuming the existence of a coding scheme for the $T$-user multiple access channel that achieves the finite block length(FBL) bounds in \cite{polyanskiy2017perspective}. The curve labelled 4-fold ALOHA is the performance of the 4-fold ALOHA scheme from \cite{ordentlich2017low} which also assumes exactly the same code. It can be seen that for large values of $\Ka$, our proposed scheme with $T=4$ substantially outperforms the 4-fold ALOHA and this gain is due to the SIC. The curve labelled OP-Exact is a reproduction of the results from \cite{ordentlich2017low} of the practical scheme introduced there. The x mark represents our proposed scheme where for the channel coding part instead of the FBL bounds we use the actual simulation results. We use a rate-1/4 $(364,91)$ LDPC code obtained from repeating every coded bit of (3,6) LDPC code twice and a message passing decoder for $T=2$. It can be seen that the simulation results with the $(3,6)$ LDPC code are only 0.5~dB away from the curve corresponding to $T=2$ showing that the pragmatic coding scheme can perform close to the finite length bounds. It can also be seen that our proposed scheme provides substantial gain over the results in \cite{ordentlich2017low}. The performance of OP-Exact is already substantially better than many other multiple access schemes and our proposed scheme can potentially provide more than 14~dB improvement over OP-Exact for large values of $\Ka$ and is only about 7~dB away from Polyanskiy's FBL bound \cite{polyanskiy2017perspective}. The slope of the $T=4$ curve also is much closer to the finite block length bound which is encouraging for larger values of $K_a$. Further details about the simulation set up can be found in \cite{avinash2017unsourcedma}.

In the proposed encoding scheme, for $L(x)=\lambda x+(1-\lambda)x^2$ each user may transmit once or twice depending on the message index chosen. We need to point out that the power constraint employed is an average over all the message indices i.e $\mathbb{E}_{w}\left[||\tilde{\vec{c}}_w||_2^2\right]=(2-\lambda)P.$
%We also present the results when the power constraint is uniform across all the codewords in the code. Fig. XXX

\ifjournal
\subsection*{Further comments:}
\begin{enumerate}
\item In bounding the error probability of GMAC decoder in Eqn. \eqref{eqn:PrFBL_sims} we employ the finite blocklength bounds instead of the actual simulations using the SCLDPC codes as described in encoding section. As we can see from Fig. \ref{fig:BP_simulations} these family of codes at moderate blocklengths $8\times 10^3-10^5$ under the computationally efficient parallel BP decoder have performance very close to the Shannon limit. But as widely known these codes are not the best choice of codes at the blocklengths in consideration for the problem i.e., $\approx 300-1000$.
\item In the proposed encoding scheme, for $L(x)=\lambda x+(1-\lambda)x^2$ each user may transmit once or twice depending on the message index chosen. We need to point out that the power constraint employed is an average over all the message indices i.e $\mathbb{E}_{w}\left[||\tilde{\vec{c}}_w||_2^2\right]=(2-\lambda)P$.
\end{enumerate}
\fi

\begin{figure}[h]
\centering
 \resizebox{0.4\textwidth}{!}{\input{../../Figures/sim_results_30000_0.04_0.01.tex}}
  \caption{Minimum $E_b/N_0$ required as a function of number of users. For the cases $ T=2,4$ and the $4$-fold ALOHA, the choices chosen for $\epsilon_0=0.04$ and $\epsilon=0.05$.}
 % and fraction of users not recovered$\leq 0.04$ given the T-user CS and GMAC channel decoding is successful at all the slots with atleast a probability of $0.99$ thus giving us the total $\Pr_e\leq 1- 0.96*0.99\approx 0.05(=\epsilon)$.}
  \label{fig:simulationresults30000}
\end{figure}

\ifjournal
\begin{figure}[h]
  \centering
  \resizebox{0.5\textwidth}{!}{\input{../../Figures/SCLDPC_two_users.tex}}
  \caption{Simulation results for two user Gaussian MAC channel where both the users employ the same codebook but implement randomly and independently chosen cyclic-shift values $\tau_{w_1}, \tau_{w_2}$ via Spatially Coupled LDPC Codes. The SC parameters are $L=16, w=3$ which incurs us a rate-loss. For instance for the rate-$1/2$ $(3,6)$ family of codes the rate-loss is $0.0625$ . The mutual information for the two-user GMAC channel is also plotted (accounting for rate-loss is also included).}
  \label{fig:BP_simulations}
\end{figure}
\fi 
